SparseZipper: Enhancing Matrix Extensions to Accelerate SpGEMM on CPUs

The importance of general matrix multiplication (GEMM) is motivating new instruction set extensions for multiplying dense matrices in almost all contemporary ISAs, and these extensions are often implemented using high-performance systolic arrays. However, matrices in emerging workloads are not always dense, and sparse matrices where the vast majority of values are zeros are becoming more common. Existing matrix extensions and micro-architectures cannot efficiently process highly sparse matrices due to two reasons: (1) wasted work when one or both input values are zero; and (2) incompatibility with sparse matrix formats. This work proposes SparseZipper that minimally modifies existing matrix extensions and systolic-array-based micro-architectures specialized for dense-dense GEMM to accelerate sparse-sparse GEMM operating on highly sparse matrices with unstructured sparsity structures. Our performance evaluation shows SparseZipper achieves 5.98x and 2.61x speedup over a scalar hash-based implementation of SpGEMM and a state-of-the-art vectorized SpGEMM version, respectively. Our component-level area evaluation shows SparseZipper increases the area of a baseline 16x16 systolic array by only 12.7% resulting in an area overhead for an entire system-on-chip of just a few percent.

==> fig-csr-format.tex <==
\begin{figure}[tp]
    \centering
    \includegraphics[width=0.7\cw]{csr_format.svg.pdf}
    \caption[Compressed Sparse Row Format]{
      \textbf{Compressed Sparse Row Format}
    }
    \label{fig-spz-csr-format}
\end{figure}


==> fig-esc-algorithm.tex <==
\begin{figure}[tp]
    \centering
    \includegraphics[width=\cw]{esc_algorithms.svg.pdf}
    \caption[Expand-Sort-Compress Algorithm]{
      \textbf{Expand-Sort-Compress Algorithm with the Block Size of Two Rows} --
      Non-zero elements are colored in the input and output matrices.
      Zero elements are left blank.
      A block of two adjacent rows in the matrix A and their corresponding rows
      in the matrix B are expanded, sorted, and compressed together to generate
      output values for the two rows in the output matrix C.
      All rows involved in the current computation step are shown within the
      dark borders.
    }
    \label{fig-spz-esc-algorithm}
\end{figure}


==> fig-example.tex <==
%=========================================================================
% fig-example.tex
%=========================================================================
% Place figure code in a separate file to make body text in the section
% files easier to read, and to simplify moving around figures.

\begin{figure}

  \includegraphics[width=0.5\tw]{example.svg.pdf}

  \caption{\textbf{Example Figure Title --} \normalfont{Descriptive text
      which usually also describes any acronyms used in the figure.}}
  \label{fig-example}

\end{figure}



==> fig-gemm-systolic-array.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\cw]{gemm-systolic-array.svg.pdf}
    \caption[Baseline Systolic Array for Accelerating Dense GEMM]{
      \textbf{A Baseline Systolic Array Micro-architecture for Accelerating
      Dense GEMM} -- PE~=~processing element.
    }
    \label{fig-spz-gemm-systolic-array}
\end{figure}


==> fig-matrix-inst-encoding.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\cw]{matrix-inst-encoding.svg.pdf}
    \caption[Matrix Instruction Encoding]{
      \textbf{Matrix Instruction Encoding} --
    }
    \label{fig-spz-mtx-inst-encoding}
\end{figure}


==> fig-mssort-code.tex <==
%=============================================================================
% asm code for sorting chunks of VL elements
%=============================================================================

%\lstset{language=[RISC-V]{Assembler}}
\lstset{style=riscv-asm-style}

\begin{figure}[tp]

  \centering
  \includegraphics[width=0.9\cw]{stream-sort-example.svg.pdf}

\begin{lstlisting}[xleftmargin=0.025\tw]
# a0, a1: base address of input key and value arrays
# a2, a3: base address of output key and value arrays
# v0, v1: lengths of the 1st and 2nd input chunks
# v2, v3: pointers to the 1st and 2nd input chunks
# v4, v5: lengths of the 1st and 2nd output chunks
# v6, v7: pointers to the 1st and 2nd output chunks
# v8, v9: index of the current set of chunk pairs and the numbers of chunk pairs
loop:
  # load
  mlxe.t tr0, 0(a0), v2, v0   # load keys of the 1st input chunks
  mlxe.t tr1, 0(a1), v2, v0   # load values of the 1st input chunks
  mlxe.t tr2, 0(a0), v3, v1   # load keys of the 2nd input chunks
  mlxe.t tr3, 0(a1), v3, v1   # load values of the 2nd input chunks
  # sort
  mssortk.tt tr0, tr2, v0, v1 # sort keys of the 1st and 2nd input chunks
  mssortv.tt tr1, tr3, v0, v1 # sort values of the 1st and 2nd input chunks
  mmv.vo v4, 0x0              # get lengths of the 1st output chunks
  mmv.vo v5, 0x1              # get lengths of the 2nd output chunks
  # store
  msxe.t tr0, 0(a2), v6, v4   # store keys of the 1st output chunks
  msxe.t tr1, 0(a3), v6, v4   # store values of the 1st output chunks
  msxe.t tr2, 0(a2), v7, v5   # store keys of the 2nd output chunks
  msxe.t tr3, 0(a3), v7, v5   # store values of the 2nd output chunks
  # check if we finish all pairs
  vadd.vx v8, v8, 0x2
  vmsltu.vv v10, v8, v9
  vpopc.m a4, v10
  bnez a4, loop
\end{lstlisting}

\caption[Sorting Chunks of Keys and Values from Multiple Streams in Parallel]{
  \BF{Sorting Chunks of Keys and Values from Multiple Streams in Parallel
  Using the Proposed Matrix Instructions} --
  This code snippet only shows the most inner loop that iterating through the
  working set of chunks bordered by the dash lines.
  VL~=~vector length;
  \TT{a\{0..4\}}~=~scalar registers;
  \TT{v\{0..9\}}~=~vector registers;
  \TT{tr\{0..3\}}~=~matrix registers.
}
\label{fig-spz-mssort-code}
\end{figure}


==> fig-mssortk-systolic-exec-example.tex <==
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\tw]{mssortk-systolic-exec-example.svg.pdf}
    \caption[Cycle-by-Cycle Systolic Execution of \TT{mssortk} in a 3$\times$3 Systolic Array for Two Unsorted Lists of Keys]{
      \textbf{Cycle-by-Cycle Systolic Execution of \TT{mssortk} in a 3$\times$3 Systolic Array for Two Unsorted Lists of Keys} --
      PE states: F~=~forward, X~=~switch, C~=~combine;
      W\_IC~=~west input counter;
      N\_IC~=~north input counter;
      E\_OC~=~east output counter;
      S\_OC~=~south output counter;
      d~=~duplicate key that is excluded;
      Counters in red indicate they are updated in corresponding cycles.
      PEs in gray are inactive.
      PEs in blue are zipping keys.
      PEs in purple are compressing valid output keys.
      Keys in red come from the north input.
      Keys in green come from the west input.
      Keys in west and east sides are ordered from bottom to top.
      Keys in north and south sides are ordered from left to right.
    }
    \label{fig:mssortk-systolic-exec}
\end{figure*}


==> fig-mszip-code.tex <==
%=============================================================================
% asm code for merging paritions of VL elements
%=============================================================================

%\lstset{language=[RISC-V]{Assembler}}
\lstset{style=riscv-asm-style}

\begin{figure}[tp]

\centering
\includegraphics[width=\cw]{stream-zip-example.svg.pdf}

\begin{lstlisting}[xleftmargin=0.025\tw]
# a0, a1: base address of input key and value arrays
# a2, a3: base address of output key and value arrays
# v0, v1: lengths of the 1st and 2nd input paritions
# v2, v3: pointers to the 1st and 2nd input paritions
# v4: lengths of the output chunks
# v5: pointers to the output chunks
loop:
  # load
  mlxe.t tr0, 0(a0), v2, v0  # load chunks of keys from 1st input partitions
  mlxe.t tr1, 0(a1), v2, v0  # load chunks of values from 1st input partitions
  mlxe.t tr2, 0(a0), v3, v1  # load chunks of keys of 2nd input partitions
  mlxe.t tr3, 0(a1), v3, v1  # load chunks of values of 2nd input partitions
  # zip
  mszipk.tt tr0, tr2, v0, v1 # zip keys of 1st and 2nd input chunks
  mszipv.tt tr1, tr3, v0, v1 # zip values of 1st and 2nd input chunks
  mmv.vi v6, 0x0             # get number of zipped input elements (1st chunks)
  mmv.vi v7, 0x1             # get number of zipped input elements (2nd chunks)
  mmv.vo v8, 0x0             # get number of output elements (1st part)
  mmv.vo v9, 0x1             # get number of output elements (2nd part)
  vsub.vv v0, v0, v6         # update input lengths (1st chunks)
  vsub.vv v1, v1, v7         # update input lengths (2nd chunks)
  vadd.vv v2, v2, v6         # bump input pointers (1st chunks)
  vadd.vv v3, v3, v7         # bump input pointers (2nd chunks)
  # store
  msxe.t tr0, 0(a2), v5, v8  # store keys of 1st output chunks
  msxe.t tr1, 0(a3), v5, v8  # store values of 1st output chunks
  vadd.vv v5, v5, v8         # bump output pointers
  msxe.t tr2, 0(a2), v5, v9  # store keys of 2nd output chunks
  msxe.t tr3, 0(a3), v5, v9  # store values of 2nd output chunks
  vadd.vv v5, v5, v9         # bump output pointers
  ...
  vpopc.m a4, v10   # count the number of active pairs of partitions
  bnez a4, loop
\end{lstlisting}

\caption[Zipping Partitions of Keys and Values across Multiple Streams in Parallel]{
  \BF{Zipping Partitions of Keys and Values across Multiple Streams in Parallel
  Using the Proposed Matrix Instructions} --
  VL~=~vector length (i.e., four elements in this example);
  \TT{a\{0..4\}}~=~scalar registers;
  \TT{v\{0..10\}}~=~vector registers;
  \TT{tr\{0..3\}}~=~matrix registers.
}
\label{fig-spz-mszip-code}
\end{figure}


==> fig-mszipk-systolic-exec-example.tex <==
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\tw]{mszipk-systolic-exec-example.svg.pdf}
    \caption[Cycle-by-Cycle Systolic Execution of \TT{mszipk} in a 3$\times$3 Systolic Array for Two Sorted Lists of Keys]{
      \textbf{Cycle-by-Cycle Systolic Execution of \TT{mszipk} in a 3$\times$3 Systolic Array for Two Sorted Lists of Keys} --
      PE states: F~=~forward, X~=~switch, C~=~combine;
      W\_IC~=~west input counter;
      N\_IC~=~north input counter;
      E\_OC~=~east output counter;
      S\_OC~=~south output counter;
      d~=~duplicate key that is excluded;
      x~=~unmergeable key;
      Counters in red indicate they are updated in corresponding cycles.
      PEs in gray are inactive.
      PEs in blue are merging keys.
      PEs in purple are compressing valid output keys.
      Keys in red come from the north input.
      Keys in green come from the west input.
      Keys in west and east sides are ordered from bottom to top.
      Keys in north and south sides are ordered from left to right.
    }
    \label{fig:mszipk-systolic-exec}
\end{figure*}


==> fig-mtx-base-insts.tex <==
\lstset{style=python-style}

\begin{figure*}[tp]
\centering

%%%%%%%%
% mmult.tt
%%%%%%%%

\includegraphics[width=\tw]{mmult_tt.svg.pdf}
\begin{lstlisting}[xleftmargin=0.025\tw]
integer esize = 32                           # element size in bits
integer dim   = MAX_VLEN / esize             # matrix dimension in elements
array<esize>[dim][dim] src_op_0 = TREG[ts2]  # first input matrix
array<esize>[dim][dim] src_op_1 = TREG[ts3]  # second input matrix
array<esize>[dim][dim] dst_op   = TREG[td1]  # output matrix
for i = 0 to dim-1:
  for j = 0 to dim-1:
    float tmp = float(dst_op[i][j])
    for k = 0 to dim-1:
      tmp += float(src_op_0[i][k]) * float(src_op_1[k][j])
    dst_op[i][j] = tmp
\end{lstlisting}

%%%%%%%%
% mlse.t
%%%%%%%%

\includegraphics[width=\tw]{mlse_t.svg.pdf}
\begin{lstlisting}[xleftmargin=0.025\tw]
integer esize = 32                           # element size in bits
integer dim   = MAX_VLEN / esize             # matrix dimension in elements
integer                src_op_0 = SREG[rs1]  # base address
integer                src_op_1 = SREG[rs2]  # stride
array<esize>[dim]      src_op_2 = VREG[vs3]  # row lengths
array<esize>[dim][dim] dst_op   = TREG[td1]  # output matrix
for row = 0 to dim-1:
  integer addr = src_op_0 + row * src_op_1
  integer rlen = min(dim, src_op_2[row])
  for col = 0 to rlen-1:
    dst_op[row][col] = MEM[addr + col * esize]
\end{lstlisting}

%%%%%%%%
% msse.t
%%%%%%%%

\includegraphics[width=\tw]{msse_t.svg.pdf}
\begin{lstlisting}[xleftmargin=0.025\tw]
integer esize = 32                           # element size in bits
integer dim   = MAX_VLEN / esize             # matrix dimension in elements
integer                src_op_0 = SREG[rs1]  # base address
integer                src_op_1 = SREG[rs2]  # stride
array<esize>[dim]      src_op_2 = VREG[vs3]  # row lengths
array<esize>[dim][dim] src_op_3 = TREG[ts1]  # input matrix
for row = 0 to dim-1:
  integer addr = src_op_0 + row * src_op_1
  integer rlen = min(dim, src_op_2[row])
  for col = 0 to rlen-1:
    MEM[addr + col * esize] = src_op_3[row][col]
\end{lstlisting}

\caption[Matrix Instructions in the Base Matrix ISA]{
  \textbf{Syntax, Encodings, and Semantics of Instructions in the Base Matrix ISA} --
  SREG~=~scalar registers;
  VREG~=~vector registers;
  TREG~=~matrix registers;
  MEM~=~memory.
}
\label{fig:spz-base-mtx-insts}
\end{figure*}


==> fig-mtx-indexed-ld-st-insts.tex <==
\lstset{style=python-style}

\begin{figure*}[tp]
\centering

%%%%%%%%
% mlxe.t
%%%%%%%%

\includegraphics[width=\tw]{mlxe_t.svg.pdf}
\begin{lstlisting}[xleftmargin=0.025\tw]
integer esize = 32                           # element size in bits
integer dim   = MAX_VLEN / esize             # matrix dimension in elements
integer                src_op_0 = SREG[rs1]  # base address
array<esize>[dim]      src_op_1 = VREG[vs2]  # index
array<esize>[dim]      src_op_2 = VREG[vs3]  # partition lengths
array<esize>[dim][dim] dst_op   = TREG[td1]  # output matrix
for row = 0 to dim-1:
  integer addr = src_op_0 + src_op_1[row]
  integer rlen = min(dim, src_op_2[row])
  for col = 0 to rlen-1:
    dst_op[row][col] = MEM[addr + col * esize]
\end{lstlisting}

%%%%%%%%
% msxe.t
%%%%%%%%

\includegraphics[width=\tw]{msxe_t.svg.pdf}
\begin{lstlisting}[xleftmargin=0.025\tw]
integer esize = 32                           # element size in bits
integer dim   = MAX_VLEN / esize             # matrix dimension in elements
integer                src_op_0 = SREG[rs1]  # base address
array<esize>[dim]      src_op_1 = VREG[vs2]  # index
array<esize>[dim]      src_op_2 = VREG[vs3]  # partition lengths
array<esize>[dim][dim] src_op_3 = TREG[ts1]  # input matrix
for row = 0 to dim-1:
  integer addr = src_op_0 + row * src_op_1
  integer rlen = min(dim, src_op_2[row])
  for col = 0 to rlen-1:
    MEM[addr + col * esize] = src_op_3[row][col]
\end{lstlisting}

\caption[Indexed Memory Instructions in SparseZipper]{
  \textbf{Syntax, Encodings, and Semantics of Indexed Load/Store Instructions in SparseZipper} --
  SREG~=~scalar registers;
  VREG~=~vector registers;
  TREG~=~matrix registers;
  MEM~=~memory.
}
\label{fig:spz-indexed-ld-st-insts}
\end{figure*}


==> fig-mtx-mssortk-inst.tex <==
\lstset{style=python-style}

\begin{figure*}[tp]
\centering

%%%%%%%%
% mssortk.tt
%%%%%%%%

\includegraphics[width=\tw]{mssortk_tt.svg.pdf}
\begin{lstlisting}[xleftmargin=0.025\tw]
integer esize = 32                          # element size in bits
integer dim   = MAX_VLEN / esize            # matrix dimension in elements
array<esize>[dim][dim] src_op_0 = TREG[ts1] # 1st input matrix
array<esize>[dim][dim] src_op_1 = TREG[ts2] # 2nd input matrix
array<esize>[dim]      src_op_2 = VREG[vs1] # lengths of 1st input chunks
array<esize>[dim]      src_op_3 = VREG[vs2] # lengths of 2nd input chunks
array<esize>[dim][dim] dst_op_0 = TREG[td1] # 1st output matrix
array<esize>[dim][dim] dst_op_1 = TREG[td2] # 2nd output matrix
# input-output index maps to be produced
array<map<integer,integer>>[dim] idx_map_0
array<map<integer,integer>>[dim] idx_map_1

for i = 0 to dim-1:
  integer inp_len_0 = min(dim, src_op_2[i])
  integer inp_len_1 = min(dim, src_op_3[i])
  # insert keys into ordered sets
  set<esize> key_set_0
  set<esize> key_set_1
  key_set0.insert(src_op_0[i][0:inp_len_0])
  key_set1.insert(src_op_1[i][0:inp_len_1])
  # update index maps
  for j = 0 to inp_len_0:
    idx_map_0[i].insert(j, key_set_0.index(src_op_0[i][j]))
  for j = 0 to inp_len1:
    idx_map_1[i].insert(j, key_set_1.index(src_op_1[i][j]))
  # update counter vectors
  integer out_len_0 = key_set_0.size()
  integer out_len_1 = key_set_1.size()
  OC0[i] = out_len_0
  OC1[i] = out_len_1
  # update dst_op
  dst_op_0[i][0:out_len_0] = key_set_0[0:out_len_0]
  dst_op_1[i][0:out_len_1] = key_set_1[0:out_len_1]
\end{lstlisting}

\caption[Stream Key Sorting Instruction in SparseZipper]{
  \textbf{Syntax, Encoding, and Semantic of \TT{mssortk.tt} Instruction in SparseZipper} --
  SREG~=~scalar registers;
  VREG~=~vector registers;
  TREG~=~matrix registers;
  MEM~=~memory;
  OC*~=~output counter vector registers;
  \TT{set}~=~data structure storing an ordered list of unique values;
  \TT{map}~=~key-value map data structure.
}
\label{fig:spz-mssortk-inst}
\end{figure*}


==> fig-mtx-mssortv-inst.tex <==
\lstset{style=python-style}

\begin{figure*}[tp]
\centering

%%%%%%%%
% mssortv.tt
%%%%%%%%

\includegraphics[width=\tw]{mssortv_tt.svg.pdf}
\begin{lstlisting}[xleftmargin=0.025\tw]
integer esize = 32                          # element size in bits
integer dim   = MAX_VLEN / esize            # matrix dimension in elements
array<esize>[dim][dim] src_op_0 = TREG[ts1] # 1st input matrix
array<esize>[dim][dim] src_op_1 = TREG[ts2] # 2nd input matrix
array<esize>[dim]      src_op_2 = VREG[vs1] # lengths of 1st input chunks
array<esize>[dim]      src_op_3 = VREG[vs2] # lengths of 2nd input chunks
array<esize>[dim][dim] dst_op_0 = TREG[td1] # 1st output matrix
array<esize>[dim][dim] dst_op_1 = TREG[td2] # 2nd output matrix
# input-output index map produced by last mssortk.tt
array<map<integer,integer>>[dim] idx_map_0
array<map<integer,integer>>[dim] idx_map_1

for i = 0 to dim-1:
  integer out_len_0 = OC0[i] # 1st output chunk's length produced by last mssortk.tt
  integer out_len_1 = OC1[i] # 2nd output chunk's length produced by last mssortk.tt
  # initialize dst_op
  for j = 0 to out_len_0:
    dst_op_0[i][j] = float(0)
  for j = 0 to out_len_1:
    dst_op_1[i][j] = float(0)
  # update dst_op
  integer inp_len_0 = min(dim, src_op_2[i])
  integer inp_len_1 = min(dim, src_op_3[i])
  for j = 0 to inp_len_0:
    out_idx = idx_map_0[i][j]
    dst_op_0[i][out_idx] += float(src_op_0[i][j])
  for j = 0 to inp_len_1:
    out_idx = idx_map_1[i][j]
    dst_op_1[i][out_idx] += float(src_op_1[i][j])
\end{lstlisting}

\caption[Stream Value Sorting Instruction in SparseZipper]{
  \textbf{Syntax, Encoding, and Semantic of \TT{mssortv.tt} Instruction in SparseZipper} --
  SREG~=~scalar registers;
  VREG~=~vector registers;
  TREG~=~matrix registers;
  MEM~=~memory;
  OC*~=~output counter vector registers;
  \TT{map}~=~key-value map data structure.
}
\label{fig:spz-mssortv-inst}
\end{figure*}


==> fig-mtx-mszipk-inst.tex <==
\lstset{style=python-style}

\begin{figure*}[tp]
\centering

%%%%%%%%
% mszipk.tt
%%%%%%%%

\includegraphics[width=\tw]{mszipk_tt.svg.pdf}
\begin{lstlisting}[xleftmargin=0.025\tw]
integer esize = 32                          # element size in bits
integer dim   = MAX_VLEN / esize            # matrix dimension in elements
array<esize>[dim][dim] src_op_0 = TREG[ts1] # 1st input matrix
array<esize>[dim][dim] src_op_1 = TREG[ts2] # 2nd input matrix
array<esize>[dim]      src_op_2 = VREG[vs1] # lengths of 1st input chunks
array<esize>[dim]      src_op_3 = VREG[vs2] # lengths of 2nd input chunks
array<esize>[dim][dim] dst_op_0 = TREG[td1] # 1st output matrix
array<esize>[dim][dim] dst_op_1 = TREG[td2] # 2nd output matrix
# input-output index maps to be produced
array<map<integer,integer>>[dim] idx_map_0
array<map<integer,integer>>[dim] idx_map_1

for i = 0 to dim-1:
  integer inp_len_0 = min(dim, src_op_2[i])
  integer inp_len_1 = min(dim, src_op_3[i])
  set<esize> key_set  # ordered set of keys from both streams
  IC0[i] = 0          # initialize 1st input counter
  IC1[i] = 0          # initialize 2nd input counter
  # insert keys into the ordered set
  for j = 0 to inp_len_0:
    if (src_op_0[i][j] <= src_op_1[i][inp_len_1]):
      key_set.insert(src_op_0[i][j])
      IC0[i] += 1
  for j = 0 to inp_len_1:
    if (src_op_1[i][j] <= src_op_0[i][inp_len_0]):
      key_set.insert(src_op_1[i][j])
      IC1[i] += 1
  # update index maps
  for j = 0 to inp_len_0:
    idx_map_0[i].insert(j, key_set.index(src_op_0[i][j]))
  for j = 0 to inp_len_1:
    idx_map_1[i].insert(j, key_set.index(src_op_1[i][j]))
  # update dst_op and output counter vectors
  integer out_len_0 = key_set.size() if (key_set.size() <= dim) else dim
  integer out_len_1 = 0 if (key_set.size() <= dim) else (dim - key_set.size())
  for j = 0 to out_len_0:
    dst_op_0[i][j] = key_set[j]
  for j = 0 to out_len_1:
    dst_op_1[i][j] = key_set[out_len_0 + j]
  # update output counter vectors
  OC0[i] = out_len_0
  OC1[i] = out_len_1
\end{lstlisting}

\caption[Stream Key Zipping Instruction in SparseZipper]{
  \textbf{Syntax, Encoding, and Semantic of \TT{mszipk.tt} Instruction in SparseZipper} --
  SREG~=~scalar registers;
  VREG~=~vector registers;
  TREG~=~matrix registers;
  MEM~=~memory;
  IC*~=~input counter vector registers;
  OC*~=~output counter vector registers;
  \TT{set}~=~data structure storing an ordered list of unique values;
  \TT{map}~=~key-value map data structure.
}
\label{fig:spz-mszipk-inst}
\end{figure*}


==> fig-mtx-mszipv-inst.tex <==
\lstset{style=python-style}

\begin{figure*}[tp]
\centering

%%%%%%%%
% mszipv.tt
%%%%%%%%

\includegraphics[width=\tw]{mszipv_tt.svg.pdf}
\begin{lstlisting}[xleftmargin=0.025\tw]
integer esize = 32                          # element size in bits
integer dim   = MAX_VLEN / esize            # matrix dimension in elements
array<esize>[dim][dim] src_op_0 = TREG[ts1] # 1st input matrix
array<esize>[dim][dim] src_op_1 = TREG[ts2] # 2nd input matrix
array<esize>[dim]      src_op_2 = VREG[vs1] # lengths of 1st input chunks
array<esize>[dim]      src_op_3 = VREG[vs2] # lengths of 2nd input chunks
array<esize>[dim][dim] dst_op_0 = TREG[td1] # 1st output matrix
array<esize>[dim][dim] dst_op_1 = TREG[td2] # 2nd output matrix
# input-output index map produced by last mszipk.tt
array<map<integer,integer>>[dim] idx_map_0
array<map<integer,integer>>[dim] idx_map_1

for i = 0 to dim-1:
  # initialize dst_op
  integer out_len_0 = OC0[i]
  integer out_len_1 = OC1[i]
  integer out_len   = out_len_0 + out_len_1
  # initialize a temporary array for accumulating values
  array<esize>[out_len] accum_arr
  for j = 0 to out_len - 1:
    accum_arr[j] = float(0)
  # update accum_arr
  for j = 0 to inp_len_0:
    out_idx = idx_map_0[i][j]
    accum_arr[out_idx] += float(src_op_0[i][j])
  for j = 0 to inp_len_1:
    out_idx = idx_map_1[i][j]
    accum_arr[out_idx] += float(src_op_1[i][j])
  # update dst_op
  for j = 0 to out_len_0 - 1:
    dst_op_0[i][j] = accum_arr[j]
  for j = 0 to out_len_1 - 1:
    dst_op_1[i][j] = accum_arr[out_len_0 + j]
\end{lstlisting}

\caption[Stream Value Zipping Instruction in SparseZipper]{
  \textbf{Syntax, Encoding, and Semantics of \TT{mszipv.tt} Instruction in SparseZipper} --
  SREG~=~scalar registers;
  VREG~=~vector registers;
  TREG~=~matrix registers;
  MEM~=~memory;
  IC*~=~input counter vector registers;
  OC*~=~output counter vector registers;
  \TT{map}~=~key-value map data structure.
}
\label{fig:spz-mszipv-inst}
\end{figure*}


==> fig-mtx-mv-insts.tex <==
\lstset{style=python-style}

\begin{figure*}[tp]
\centering

%%%%%%%%
% mmv.vi
%%%%%%%%

\includegraphics[width=\tw]{mmv_vi.svg.pdf}
\begin{lstlisting}[xleftmargin=0.025\tw]
integer esize = 32                    # element size in bits
integer dim   = MAX_VLEN / esize      # matrix dimension in elements
integer src_imm           = cimm      # counter vector index
array<esize>[dim] dst_op  = VREG[vd]  # output vector
for i = 0 to dim-1:
  dst_op[i] = IC0[i] if src_imm == 0 else IC1[i]  # copy from output counter vector reg
\end{lstlisting}

%%%%%%%%
% mmv.vo
%%%%%%%%

\includegraphics[width=\tw]{mmv_vo.svg.pdf}
\begin{lstlisting}[xleftmargin=0.025\tw]
integer esize = 32                    # element size in bits
integer dim   = MAX_VLEN / esize      # matrix dimension in elements
integer           src_imm = cimm      # counter vector index
array<esize>[dim] dst_op  = VREG[vd]  # output vector
for i = 0 to dim-1:
  dst_op[i] = OC0[i] if src_imm == 0 else OC1[i]  # copy from output counter vector reg
\end{lstlisting}

\caption[Counter Vector Move Instructions in SparseZipper]{
  \textbf{Syntax, Encoding, and Semantics of Counter Vector Move Instructions in SparseZipper} --
  VREG~=~vector registers;
}
\label{fig:spz-mtx-mv-insts}
\end{figure*}


==> fig-plot-example.tex <==
%=========================================================================
% fig-plot-example
%=========================================================================

\begin{figure}[t]

  \includegraphics[width=\cw]{plot-example.py.pdf}

  \caption{\textbf{Example Figure Title --} \normalfont{Descriptive text
      which usually also describes any acronyms used in the plot.}}
  \label{fig-plot-example}

\end{figure}



==> fig-result-hit-rate.tex <==
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\tw]{plot-spz-l1d-hit-rate.svg.pdf}
    \caption[L1 Data Cache Hit Rate in SparseZipper]{
      L1 Data Cache Hit Rate
    }
    \label{fig-spz-result-hit-rate}
    \vspace{-0.3cm}
\end{figure*}


==> fig-spa-algorithm.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\cw]{spa-algorithm.svg.pdf}
    \caption[SpGEMM Algorithm Using Dense Array for Accumulating Sparse Values]{
      \BF{Array-Based SpGEMM Algorithm}
    }
    \label{fig-spz-spa-algorithm}
\end{figure}


==> fig-sparse-zipper-o3-pipeline.tex <==
\begin{figure}[tp]
    \centering
    \includegraphics[width=0.35\cw]{sparse-zipper-o3-pipeline.svg.pdf}
    \caption[Out-Of-Order Core Pipeline with an Integrated Systolic Array]{
      \textbf{Out-Of-Order Core Pipeline with an Integrated Systolic Array for Executing Matrix Instructions}
    }
    \label{fig:spz-sparse-zipper-o3-pipeline}
\end{figure}


==> fig-spgemm-dataflows.tex <==
\begin{figure}[tp]
    \centering
    \includegraphics[width=\cw]{spgemm_dataflows.svg.pdf}
    \caption[Different Sparse GEMM Dataflows]{
      \textbf{Different SpGEMM Dataflows} -- Non-zero elements in the input
      matrices (i.e., A and B) and the output matrix (i.e., C) are colored.
      Zero elements are left blank. In each computation step, involved matrix
      elements are shown within the dark borders.
    }
    \label{fig-spz-spgemm-dataflows}
\end{figure}


==> sec-background-mtx-arch.tex <==
%-------------------------------------------------------------------------
% Background on matrix extensions
%-------------------------------------------------------------------------

\section{Background: Modern Matrix Architectures}
\label{sec-spz-mtx-ext-background}

\input{fig-gemm-systolic-array}

% dedicated matrix-multiply accelerators
The ever-growing importance of GEMM performance and efficiency in emerging
workloads such as machine learning has driven architects to design and
integrate accelerators for dense GEMM in modern systems.
For example, Google introduced its Tensor Processing Unit (TPU) as a
co-processor next to a general-purpose CPU for accelerating training and
inference kernels in machine learning
workloads~\cite{jouppi-datacenter-isca2017,teich-google-tpu-v2-blog2018,jouppi-google-tpu-v2-v3-cacm2020,jouppi-tpu-v4-isca2023}.
At the heart of TPU is a large matrix-matrix multiply unit that significantly
improves the performance and energy efficiency of multiplying two dense
matrices compared to contemporary CPUs and GPGPUs.
NVIDIA also integrates tensor cores specialized for multiplying and adding
matrices in its recent GPUs~\cite{choquette-nvidia-tensor-core-2021}.

% instruction set for matrix-multiply operation
The need for accelerating GEMM has pushed specialization for dense GEMM further
into modern general-purpose CPU instruction sets as well.
Arm recently released its Scalable Matrix Extension (SME) that introduces a new
instruction performing an outer product of two vectors and accumulating its
results into a new two-dimensional accumulator register
state~\cite{arm-sme-web}.
IBM took a similar approach in its Matrix-Multiple Assist (MMA) extension for
the Power ISA~\cite{ibm-mmx-assist-web}.
Intel introduced a new Advanced Matrix Extension (AMX) that adds several
two-dimensional matrix register states called tile registers and a new
matrix-matrix multiply instruction performing a matrix multiplication on two
input tile registers~\cite{intel-amx-web,nassif-intel-sapphire-isscc2022}.
The RISC-V community is also working on a matrix extension
proposal~\cite{riscv-mtx-ext-proposal-web} that is similar to Intel AMX's
approach.

% micro-architecture
Regardless of programming abstractions (e.g., accelerator-based interfaces and
instruction sets), specialization for dense GEMM is typically implemented in
hardware using a two-dimensional systolic array consisting of multiply-add
processing elements
(PEs)~\cite{jouppi-datacenter-isca2017,jeong-rasa-dac2021,nassif-intel-sapphire-isscc2022}.
An implementation of a systolic array can be either input-, weight-, or
output-stationary (i.e., which input/output matrix stays inside the systolic
array throughout the computation), depending on its programming abstraction.
The integration of a matrix-multiply unit and a general-purpose CPU can be
either coarse-grained (e.g., as a co-processor like TPU), medium-grained (e.g.,
sharing some levels of caches with the CPU), or fine-grained (e.g., as a
functional unit in the CPU's pipeline).

% explain the baseline micro-architecture
Figure~\ref{fig-spz-gemm-systolic-array} shows a weight-stationary systolic
array for accelerating dense GEMM.
The array consists of multiple PEs connected in a two-dimensional mesh network.
Each PE receives input data from its west and north input ports, sends
output value (i.e., partial sum of an output matrix element) to its south
neighbor PE, and forwards input data to its east neighbor PE.
Each PE consists of a weight register for keeping weight values that are
multiplied with input values over multiple iterations in a weight-stationary
GEMM implementation.
In addition, a multiply-accumulate (MAC) unit is used to multiply a weight
value (i.e., in the weight register) with an input value (i.e., from the west
input port) and accumulate the result into an output value (i.e., from the
north input port).
There are skew buffers in the west and north input ports so that input data are
staggered in time when entering the systolic array.


==> sec-background-spgemm.tex <==
%=========================================================================
% SparseZipper: Background
%=========================================================================

%-------------------------------------------------------------------------
% Background on SpGEMM
%-------------------------------------------------------------------------
% Take-aways:
%   - Row-wise dataflow is efficient (time and space) and parallelizable
%   - Different ways to implement the row-wise product dataflow
%       + Using an accumulator
%       + Using ESC method

\section{Background: Sparse General Matrix Multiplication}
\label{sec-spz-spgemm-background}

Sparse general matrix multiplication (SpGEMM) is a commonly used building block
in various application domains including graph
analytics~\cite{davis-graphblas-tmos2019,hoefler2011generic,shun-multicore-tc-2015},
machine
learning~\cite{reddi-mlperf-isca2020,naumov-dnn-model-arxiv2019,han-deep-compress-arxiv2015,jouppi-datacenter-isca2017,wu-ml-facebook-hpca2019},
and scientific computing~\cite{canning-sparse-sim-1996,galli-quantum-sim-1996}.
This section describes widely used data structures for representing sparse
matrices, various algorithms for multiplying two sparse matrices, and their
trade-offs.

%----------
% Matrix formats
%----------

\subsection{Sparse Matrix Formats}
\input{fig-csr-format}

Since most elements in a sparse matrix are zeros, it is efficient to store only
non-zero elements to minimize the amount of required storage and also avoid
ineffectual computation (i.e., multiplying with zero).
The most common data structures for storing a sparse matrix are coordinate
format (COO), compressed sparse row (CSR), and compressed sparse column (CSC).
They are the default data structures in many widely used linear algebra
libraries such as Intel Math Kernel Library (MKL)~\cite{wang-intel-mkl-2014},
CUSPARSE~\cite{naumov-cusparse-2010}, and
Matlab~\cite{gilbert-sparse-matlab-1992}.

COO format stores a list of tuples including row index, column index, and value
of non-zero elements in a sparse matrix.
Typically, the list is kept sorted by either row indices, column indices, or a
combination of both row and column indices for more efficient lookups and
memory accesses.
Further improving the storage efficiency, compared to COO, CSR format groups
per-row non-zero elements so that the row indices for elements in the same row
can be further compressed.
Figure~\ref{fig-spz-csr-format} shows an example of CSR format.
Non-zero elements in each row are represented by a stream of keys (i.e., column
indices) and values (i.e., element data).
Typically, elements in a stream are sorted by their keys, and streams of
adjacent rows are placed consecutively in memory to form the column index and
value arrays.
The row pointer array consists of pointers indicating where each row starts in
the column index and value arrays.
CSC format is similar to CSR format except that non-zero elements are
compressed by columns.

In addition to those general sparse matrix formats, there are numerous
other sparse matrix formats specialized for certain structures of non-zero
elements and/or
target architectures~\cite{borvstnik-dbcsr-2014,hu-graphlily-iccad2021,gomez-spmv-vector-2021,srivastava-matraptor-micro2020,chen-spgemm-taihulight-2018}.
However, such specialized matrix formats often incur format converting
overheads, and their performance is not portable across different matrices and
architectures.
In this chapter, we assume CSR/CSC which are storage-efficient and widely used
sparse matrix formats.

%----------
% Dataflows
%----------

\input{fig-spgemm-dataflows}
\subsection{SpGEMM Dataflows}

Figure~\ref{fig-spz-spgemm-dataflows} shows common dataflows for SpGEMM:
inner-product, outer-product, and row-wise-product (also known as Gustavson's
algorithm).

\BF{Inner-product dataflow --}
This dataflow computes each element in the output matrix one at a time by doing
a dot product between two vectors (i.e., a row in matrix A and a corresponding
column in matrix B), as shown in Figure~\ref{fig-spz-spgemm-dataflows}.
Since there is no data dependency among output elements, the inner-product
dataflow is highly parallelizable by computing multiple dot products for
different output elements in parallel.
In addition, this dataflow also has good data locality for the output matrix
but low data reuse for the input matrices.
One major downside of this approach is the inefficiency of doing a dot product
between two sparse vectors.
Since input matrices are sparse, the output matrix is likely to have few
non-zero elements.
Therefore, most of the dot products result in zeros.
Furthermore, the dot product of two sparse vectors requires intersecting two
lists of indices, and this index matching is highly inefficient due to the high
sparsity of a row and a column in the input matrices.

\BF{Outer-product dataflow --}
Unlike the inner-product dataflow, the outer-product dataflow computes partial
results for the entire output matrix at each step by doing an outer product
between a column in matrix A and a corresponding row in matrix B, as shown in
Figure~\ref{fig-spz-spgemm-dataflows}.
Partial results are combined into a single final output matrix C.
All non-zero elements in a column in matrix A and a row in matrix B are used to
generate non-zero elements in matrix C, so the outer-product dataflow avoids
the problem of ineffectual index matching operations in the inner-product
dataflow.
Multiple outer-product operations on different pairs of matrix A's columns and
matrix B's rows can happen in parallel.
However, combining partial outer-product results typically requires complex
synchronizations, and this step is often a performance bottleneck in this
approach.
Despite having good input data reuse, the outer-product dataflow has low output
data reuse, and the aggregate memory space of all partial output matrices is
often much larger than the final output matrix's size.

\BF{Row-wise-product dataflow --}
The row-wise-product dataflow computes each row of the output matrix at a time
by multiplying a row in matrix A (sparse vector) with the entire matrix
B, as shown in Figure~\ref{fig-spz-spgemm-dataflows}.
Similar to the outer-product dataflow, this row-wise-product dataflow is
work-efficient since it processes only non-zero input elements that contribute
to generating non-zero output elements.
In each step, a multiplication between a sparse vector and a sparse matrix may
require merging some partial output vectors into a final row in the output
matrix.
However, compared to the two-dimensional matrix merging step in the
outer-product dataflow, merging partial one-dimensional sparse vectors is much
less complex and requiring much less temporary memory space, which may fit in
on-chip caches.
The row-wise-product dataflow has relatively poor data reuse of matrix B since
column indices of non-zero elements in each row in matrix A are used to access
corresponding rows in matrix B.
Finally, unlike both the inner-product and outer-product approaches, the
row-wise-product dataflow does not require input matrices to be stored in two
different formats: CSR and CSC.
All input and output matrices can be consistently stored in CSR, so there is no
need for converting between sparse matrix formats.

\input{tab-spgemm-dataflows}

Table~\ref{tab-spz-spgemm-dataflows} summarizes trade-offs among the three
SpGEMM dataflows.
In this work, we consider only the row-wise-product dataflow since it is
relatively work-efficient by avoiding the extremes in both inner-product and
outer-product dataflows.

%----------
% Row-wise algorithms
%----------

\subsection{Row-Wise Product Algorithms}

There are three common algorithms to implement the row-wise-product dataflow
for SpGEMM: array-based, hash-based, and expand-sort-compress algorithms.

\input{fig-spa-algorithm}
\BF{Array-based row-wise SpGEMM --}
This is also known as sparse accumulator algorithm
(SPA)~\cite{gilbert-sparse-matlab-1992}.
Figure~\ref{fig-spz-spa-algorithm} shows an example of how this algorithm
works.
The algorithm uses a set of three dense arrays that have the same size as the
number of columns in the output matrix.
The first two arrays store accumulated values and valid flags.
When a key-value tuple is inserted, it accesses the two arrays by the key.
If the flag for the key is false (i.e., no valid value has been added for this
key yet), it overwrites the corresponding entry in the accumulated value array
and sets the flag to true.
Otherwise, the new value is added to the existing value.
The third array stores inserted keys in the order they are first added to the
list.
Those keys are also indices to the value and flag arrays.
After all key-value tuples are inserted, we can iterate through the key array
to construct an unsorted list of key-value output list.
The list is then sorted by keys to produce one row of the output matrix.
The flag array needs to be reset before processing the next matrix row.

\BF{Hash-based row-wise SpGEMM --}
Another common approach to accumulate sparse values in row-wise SpGEMM is using
a hash table~\cite{anh-hash-spgemm-2016,deveci-multithreaded-spgemm-2018}.
Key-value tuples are inserted into a hash table based on their hashed keys.
Similar to the array-based row-wise SpGEMM, key-value tuples in the hash table
are not sorted, so a final sorting step is needed to generate an output matrix
with per-row non-zero elements sorted by their column indices.

\input{fig-esc-algorithm}
\BF{Expand-Sort-Compress (ESC) algorithm --}
ESC algorithm was initially proposed for performing SpGEMM on
GPUs~\cite{dalton-spgemm-gpu-2015,winter-adaptive-spgemm-gpu-ppopp2019} and
later adopted to vector
architectures~\cite{fevre-spgemm-rvv-2023,li-spgemm-vector-arch-mchpc2019}.
Figure~\ref{fig-spz-esc-algorithm} shows an example of how this ESC algorithm
works.
Unlike the array-based and hash-based SpGEMM algorithms, more than one row of
the input matrix A and output matrix C can be processed together to increase
the amount of work that can be parallelized or vectorized.
Intermediate results of multiplications are expanded in triples of row index,
column index, and value.
The list of triples are then sorted by their row and then column indices.
Triples with duplicate key (i.e., same row and column indices) are compressed
into one entry with the values being accumulated in the final output.


==> tab-spgemm-dataflows.tex <==
\begin{table*}[tp]
  \centering
  \cbxsetfontsize{10pt}

  \begin{tabular}{lcccccccc}
  \toprule
  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataflow}}} & \multicolumn{3}{c}{\textbf{Data Access Efficiency}}                           & \multicolumn{3}{c}{\textbf{Sparse Format}}                                    & \multicolumn{2}{c}{\textbf{Algorithmic Efficiency}} \\
  \cmidrule{2-4}  \cmidrule{5-7} \cmidrule{8-9}
  \multicolumn{1}{c}{}                                   & \textbf{Mtx A} & \multicolumn{1}{l}{\textbf{Mtx B}} & \textbf{Mtx C} & \textbf{Mtx A} & \multicolumn{1}{l}{\textbf{Mtx B}} & \textbf{Mtx C} & \textbf{Time}            & \textbf{Space}           \\
  \midrule
  Inner-product                                          & Low               & High                                  & High              & CSR               & CSC                                   & Either            & Low                      & High                     \\
  Outer-product                                          & High              & High                                  & Low               & CSC               & CSR                                   & CSR               & High                     & Low                      \\
  Row-wise-product                                       & High              & Low                                   & High              & CSR               & CSR                                   & CSR               & High                     & Medium                   \\
  \bottomrule
  \end{tabular}

  \caption[Trade-offs Among Different SpGEMM Dataflows]{
    \textbf{Trade-offs Among Different SpGEM Dataflows}
  }
  \label{tab-spz-spgemm-dataflows}

\end{table*}

